NetScatter: Enabling Large-Scale Backscatter Networks

We present the first wireless protocol that scales to hundreds of concurrent transmissions from backscatter devices. Our key innovation is a distributed coding mechanism that works below the noise floor, operates on backscatter devices and can decode all the concurrent transmissions at the receiver using a single FFT operation. Our design addresses practical issues such as timing and frequency synchronization as well as the near-far problem. We deploy our design using a testbed of backscatter hardware and show that our protocol scales to concurrent transmissions from 256 devices using a bandwidth of only 500 kHz. Our results show throughput and latency improvements of 14--62x and 15--67x over existing approaches and 1--2 orders of magnitude higher transmission concurrency.

==> acks.tex <==
\section{Acknowledgments.}
{
  We thank Suman Banerjee and Ben Ransford for their helpful feedback on the paper. This work was funded in part by awards from the National Science Foundation (CNS--1452494, CNS--1407583, CNS--1305072) and Google Faculty Research Awards.
}



==> applications.tex <==
\section{Proof-of-Concept Applications}

This paper demonstrates backscatter communication on commodity devices, and in this section we evaluate prototypes of three novel applications enabled by these techniques. We evaluate only the communication aspect of our prototypes and consider fully exploring their security and usability issues outside the of scope of this work.


\subsection{Smart Contact Lens}
Smart contact lens systems~\cite{liao20123,yao2012contact} measure biomarkers like glucose, cholesterol and sodium in tears that can help with unobtrusive tracking for diabetic patients. The lens consists of a miniature glucose sensor IC, and an antenna. Although the power required for glucose sensing is minimal, real-time communication is power consuming and rules out conventional radios. Today these systems are limited to periodically sampling and storing the glucose data that is then transmitted sporadically using backscatter whenever the lens is next to a dedicated, powered, RFID-like reader.

We leverage our design to show that a smart contact lens can communicate with commodity Wi-Fi and Bluetooth radios, without the need for dedicated reader hardware. We develop the form factor antenna prototype lens shown in Fig.~\ref{fig:rssi_contact_lens}. The prototype consists of a 1~cm diameter loop antenna similar to prior contact lens systems~\cite{liao20123, yao2012contact}. The antenna was built using 30~AWG wire and then encapsulated in a 200 $\mu$m thick layer of poly-dimethylsiloxane (PDMS) for biocompatibility and structural integrity. We then connect the antenna to our FPGA prototype. Unlike traditional antennas that have a 50 $\Omega$ impedance, small loop antennas have non-standard impedances and so we optimize the impedance of the backscatter switch network for the impedance of our loop antenna. We note that for ease of prototyping, we use FPGA hardware but an IC should conform to the contact lens size form factor, similar to prior backscattering lens designs~\cite{lens1}.

To evaluate the system, we immerse our antenna prototype in contact lens solution. We configure the TI Bluetooth chip to transmit every 40~ms and place it 12 inches from the lens. We use the Intel Wi-Fi card as a receiver and vary its distances to the lens antenna. The RSSIs follow a similar trend when using a Samsung Galaxy S4 as the receiver. We configure our FPGA to detect the Bluetooth beacons and backscatter 2~Mbps Wi-Fi packets. Fig.~\ref{fig:rssi_contact_lens} plots the Wi-Fi RSSI for different Bluetooth transmit power values. The plot shows that we can achieve ranges of more than 24~inches, demonstrating the feasibility of a smart contact lens that communicate directly with commodity radios. We note that the range is smaller than prior plots because the antenna is much smaller and is immersed in liquid leading to high signal attenuation. The range however is similar to prior smart contact lens with a dedicated RFID-like reader~\cite{lens1}.


\begin{figure}[!t]
        \subfigure
        {
          \includegraphics[width=.25\columnwidth]{./figures/contact_ant.eps}
        }
        \subfigure
        {
          \includegraphics[width=0.7\columnwidth]{./figures/contact_lens.eps}
        }
\vskip -0.1in
  \caption{{\bf RSSI with smart contact lens antenna prototype.}}
\vskip -0.15in
\label{fig:rssi_contact_lens}
\end{figure}


\subsection{Implanted Neural Recording Devices}
Implantable neural recording devices have recently demonstrated promising results towards use in brain-computer interfaces (BCIs)~\cite{leuthardt2004brain} that help paralyzed individuals operate motor prosthetic devices, command electronic devices, or even regain control of their limbs~\cite{hochberg2006neuronal}. These systems use either penetrating neural probes~\cite{bmi2} or a surface electrode grid~\cite{wyler1984subdural} that is implanted to collect local field potentials and electrocorticography (ECoG) signals~\cite{bmi2}. The recording sensors today consume around 2~$\mu$W/channel~\cite{wyler1984subdural}, with 8--64 parallel recording channels.



\begin{figure}[!t]
        \subfigure
        {
          \includegraphics[width=.25\columnwidth]{./figures/bmi_ant.eps}
        }
        \subfigure
        {
        \includegraphics[width=0.7\columnwidth]{./figures/bmi.eps}
        }
\vskip -0.1in
\caption{{\bf RSSI with implantable neural recording antenna.}}
\vskip -0.15in
\label{fig:rssi_bmi}
\end{figure}
Instead of using a custom backscatter reader as prior prototypes~\cite{bmi1,bmi2,bmi3}, we leverage our design to transmit the data directly to commodity radios. To demonstrate this, we built a form factor antenna for the implantable neural recording device shown in Fig.~\ref{fig:rssi_bmi}. We construct a 4~cm diameter full wavelength loop antenna using 16 AWG magnet wire and encapsulate it in a 2~mm thick layer of PDMS to isolate it from biological tissue.

These devices are typically implanted either on top of the dura beneath the skull or just under the skin inside the skull cavity. For our in-vitro evaluation, we choose muscle tissue whose electromagnetic properties are similar to grey matter at 2.4~GHz~\cite{gabriel1996dielectric}. We took a 0.75~inch thick pork chop and created a slit 0.0625~inch from the surface and inserted the antenna. We use the TI Bluetooth device as our RF source and place it at a distance of 3~inches from the meat surface. We use Intel Link 5300 Wi-Fi card on channel 11 as our Wi-Fi receiver; the RSSI results were similar with a Samsung S4. We set our FPGA prototype to synthesize 2~Mbps Wi-Fi packets. Fig.~\ref{fig:rssi_bmi} shows the RSSI for different Bluetooth powers. The plots show the feasibility of communicating with implanted devices, despite significant attenuation due to the muscle tissue. The range we achieve is better than the 1-2~cm target range for existing prototypes~\cite{bmi1, bmi2}. Finally, since Samsung Note 5 and iPhone 6 support 10~dBm Bluetooth transmissions, this demonstrates an implantable device that can communicate with commodity mobile devices.


\subsection{Card to Card Communication}
Finally, we can use the single-tone transmission from Bluetooth devices to enable communication between two passive cards similar to ambient backscatter~\cite{abc-sigcomm2013}, but without the need for strong TV transmissions. Since most users have Bluetooth-enabled devices (e.g., smartphone), this could be used for money transfer between credit cards, bus passes, splitting of checks, or transferring content to digital paper devices.

We prototype proof-of-concept credit card form factor devices shown in Fig.~\ref{fig:card_2_card} that backscatter the single-tone from the Bluetooth device to communicate between each other. We replicate prior work on ambient backscatter~\cite{abc-sigcomm2013} and use its receiver architecture. We however, tune the hardware to operate at 2.4~GHz instead of the UHF TV band. The prototype also has an IGLOO Nano FPGA to implement digital baseband processing for \name\, an MSP430 micro-controller for running application software, LEDs for visual feedback, an accelerometer and capacitive touch sensors for user input.

\begin{figure}[!t]
        \subfigure%[Card to Card Prototype]
        {
          \includegraphics[width=.25\columnwidth]{./figures/card_to_card.eps}
        }
        \subfigure
        {
        \includegraphics[width=0.7\columnwidth]{./figures/tag2tag.eps}
        }
\vskip -0.15in
        \caption{{\bf BER for communication between two cards with integrated antennas.} Amazon card shown for comparison.}
\vskip -0.15in
\label{fig:card_2_card}
\end{figure}

We evaluate card to card communication by configuring one card to periodically transmit an 18 bit payload at 100~kbps to another, at time instances corresponding to the single-tone Bluetooth transmissions. The cards use their energy detectors to synchronize with the Bluetooth transmissions. We place the transmit card 3~inches from a 10~dBm TI Bluetooth device and vary the location of the receiver. Fig.~\ref{fig:card_2_card} shows the bit error rate achieved. The plot demonstrates that up to a distance of 30~inches, 10~dBm Bluetooth transmissions achievable on smartphones such as the Note 5 and iPhone 6, can enable card to card communication.



==> conclusion.tex <==
re\section{Discussion and Conclusion}
We introduce a novel approach that transforms wireless transmissions from one technology to the other, on the air. Specifically, we show for the first time that Bluetooth transmissions can be used to generate Wi-Fi and ZigBee-compatible signals using backscatter communication. Using this approach, we build proof-of-concepts for previously infeasible applications including the first contact lens form-factor antenna prototype and an implantable neural recording interface that communicate directly with commodity devices such as smartphones and watches, thus enabling the vision of Internet connected implanted devices.

\textred{Finally we outline research directions for improving upon this work. First, interscatter enables high bit rates which allow data to be transmitted in shorter periods of time. This reduces the time for which transmissions occupy the channel and can reduce power consumption by duty cycling the device. Future work could improve overall throughput by using BLE data packets which can be transmitted at a faster rate than BLE advertisements. Additionally the latest Bluetooth standard increases the maximum length for these data packets which would further improve throughput. Lastly, while our current design focuses on generating 802.11b transmissions using backscatter, future work could explore OFDM based protocols such as 802.11g/n/ac to improve the bit rates we achieve by an additional order of magnitude.}


==> design.tex <==
\section{Multi-User CSS (\nameshort)}
In this section, we will go over different methods used for multi-user CSS.
\subsection{Using Different Spreading Factors}
If there are $N$ transmitters in the network, one way to enable concurrent transmissions is to assign different spreading factors to each of them. There are two fundamental  problems associated to this network. The first problem is, the receiver needs to use downchirps with different spreading factors to despread upchirp symbols of different transmitters which increases the receiver complexity. Second, upchirps with different spreading factors are not orthogonal. As shown in Fig. xx(figure with upchirps with different spreading factors and their despread version and noise contributions), if we have a signal composed of two upchirps with different spreading factors and we despread this signal using the downchirp corresponding to first upchirp, then the second upchirp will increase the noise floor of the first upchirp.(explain this part better) This will reduce the sensitivity of the receiver.  
\subsection{Multiple Concurrent Transmissions in LoRa}  
Imagine that there are two perfectly synchronized transmitters sending two different upchirp symbols as shown in Fig. xx a (two different upchirps with different colors in one figure). By superposition theorem, we will be able to see two different peaks in the FFT of the received signal shown in Fig. xx b and if we are able: 1- differentiate these peaks and 2- associate them to the corresponding transmitter we can have two concurrent transmissions at the same time. One way to differentiate between the transmitters is to use the fraction in their FFT peak indexes(cite CMU paper). However, this is limited to 10 in an ideal case and practically cannot support more than 7 concurrent transmissions. Moreover, if these two transmitters use the same upchirp symbol at the same time, it will result in a collision that cannot be decoded. In the case of LoRa modulation, if there are $N$ transmitters and assuming random symbols at each symbol time interval, the probability of collision is equal to:
\begin{equation}
P_{collision}=1-\prod_{i=1}^{N}(1-\frac{i}{2^{SF}})\simeq\frac{N(N+1)}{2^{SF+1}}
\end{equation}\par
To make sense of the above probability, assume $SF=9$ and $N=10$. Collision probability is approximately 10\% in this case. In the next section, we go over the \nameshort and explain how it will satisfy the two requirements mentioned above.


\subsection{\nameshort} 
As explained above, the previous methods of enabling multi-user CSS are problematic. If we look at the FFT plots of Fig. xx(first figure), all the frequency bins expect one bin is empty; however these empty bins can be utilized to transmit data orthogonal to other bins. Therefore, we decided to modify the CSS modulation used in LoRa protocol so that we can make use of the unused FFT bins. In particular, each tag is assigned to a particular upchirp symbol and sends data by either sending the upchirp symbol or not sending it. In other words, each tag is sending data by doing on-off keying of the its assigned upchirp symbol. As shown in Fig. xx (have 3 different full packets) all the tags have a fixed number of upchirp preamble symbols (6 in our design) and their preamble code is the same as their assigned code. After that, 2 and a quarter downchirps will be sent. Downchirps' code is the same as the tag's assigned code as well. The reason for sending different preamble upchirp and downchirp codes is to make sure that their FFT bins don't collide after demodulation and taking FFT. Then, fixed number of payload upchirp symbols will be sent. \par
In on-off keying CSS, there can be as many as $2^{SF}$ transmissions at each symbol period ideally. Compared to LoRa, this will increase bandwidth efficiency and increase throughput from $\frac{BW}{2^{SF}}SF$ to $BW$.

\section{CSS on-off keying: modulation and demodulation}
\subsection{Sensor Code Assignment and Packet Structure}
Two ways of changing code: 
-change starting frequency of baseline chirp 
-cyclically shift the baseline chirp
Explain the packet structure and how are we modulating data
\subsection{Demodulation}
Explain the high FFT size and zero-padding\par
How to find the start of the packet
\subsection{Synchronization}
how are we doing the synchronization
\subsection{Delay and Frequency offsets}
frequency offset and delay considerations => evaluation\par
BER measurement for different guard sizes => evaluation \par
We can adjust frequency offset in association phase\par
Delay can be adjusted in association phase\par
\subsection{BW Stitching}
Explain how we can stitch two or more bands and decode them at the same time












==> discussion.tex <==
\section{Discussion}


==> eval.tex <==
\section{Evaluation and Results}\label{eval}
In this section, we characterize practical issues described previously and will show the results of final implementation. 
In this section, we evaluate frequency and timing mismatches for \tagnames.

\subsection{Frequency offset (FO)} 
{\it Method.} We evaluated the frequency offset for each of \tagnames using a wired setup. For doing so, we recorded thousand packets for each of the \tagnames using a preamble that is known between the AP and \tagname in USRP. Using the method described in \xref{dl_offset}, we found the frequency offset for each \tagname. We show frequency offset for more than 50 backscatter \tagnames and also ten active \tagnames in Fig.~\ref{fig:FO}. 

{\it Results and explanations.} As explained previously, since the output frequency of the backscatter \tagname is a few MHz and knowing the crystal frequency tolerance of 50~ppm, frequency offset should be less 100s of Hz which is much less than one FFT bin and need not to be corrected. However, active \tagnames hardware has output frequency of 900~MHz and knowing crystal frequency tolerance of 10~ppm for LoRa chip in reference board SX1276RF1KAS, the frequency offset should be less than 9~KHz. This means that we need to correct for the frequency offset for active \tagnames. 

\begin{figure}[t]
	\begin{subfigure}{\columnwidth}
    	\centering
    	\includegraphics[width=\linewidth]{./figs/3_bench_passive_FO_TO/passive_FO.eps}
		\label{fig:FO_passive}
	\end{subfigure}
    \vskip -0.3in
    \begin{subfigure}{\columnwidth}
    	\centering
    	\includegraphics[width=\linewidth]{./figs/7_bench_active_FO_TO/active_FO.eps}
		\label{fig:FO_active}
	\end{subfigure}
    
\vskip -0.3in
\caption{{\bf Frequency Offset Evaluation.} We evaluate frequency offset of passive and active \tagnames.} 
\label{fig:FO}
\vskip -0.15in
\end{figure}

\subsection{ Frequency offset and Time Offset (TO)}
\label{sec:eval_TOFO}
{\it Method.} The next step to characterize the system is to look at the FFT bin variation, $\Delta FFT$, over time. This characterization will help us find out how many empty cyclic shifts (K in ~\xref{sec:timing}) we need to put for each occupied cyclic shift. The source of $\Delta FFT$ is TO and FO. This means by finding the $\Delta FFT$ we can find TO and FO as well. To do this, we setup a wireless experiment sending query packets from the AP and receiving transmissions from multiple for active and backscatter \tagnames, separately. Decoding these transmissions and comparing the received cyclic shifts with what we have programmed the \tagnames to send, we can find the $\Delta FFT$ for these transmissions for each \tagname. 

{\it Results and explanations.} Fig.~\ref{fig:FOTO} shows the frequency and timing offset for both backscatter and active \tagnames. Note that, backscatter $\Delta FFT$ is different and in our case less the active one. The reason is simply the difference between the hardwares. In backscatter \tagname, the energy detector receives the amplitude modulated query packet and sends interrupt to backscatter transmitter to initiate transmissions. The hardware delay variation in this case comes from different receiving times  

We setup our passive \tagnames in an office environment and active \tagnames on a university campus.


\begin{figure}[h]
	\centering
	\includegraphics[width=\linewidth]{./figs/1_bench_fft_variation/delay_variation.eps}
	\label{fig:sfig1}
\vskip -0.3in
\caption{{\bf FFT Bin Variation Evaluation.} This results show that by using lower chirp bandwidth, we can support more \tagnames in the same spectrum and increase network throughput.}
\label{fig:fft_var}
\end{figure}

{\it Doppler Effect.} We evaluate Doppler effect on different transmissions for our \tagnames. In theory, the effect of low speed mobile devices, which is the target of our system, is not considerable compare to other source of frequency variations. For example if a \tagname move with XX~m/s, Doppler effect would be around XXXX~Hz which is small . We evaluate frequency offset of \tagname in difference speeds. We setup an experiment where a user holds a \tagname and moves with different speed. We record transmissions from \tagname and evaluate frequency shift of each chirp symbol. As Fig.~ref{fig:doppler} shows, frequency offset plus time offset for moving scenarios with different speed is similar to static scenario.

\begin{figure}[h]
        \includegraphics[width=\columnwidth]{./figs/6_bench_doppler/bench_doppler.eps}
\vskip -0.15in
\caption{{\bf Doppler Effect Evaluation.} We evaluate Doppler effect of FO+TO in static scenario compare to moving scenario at different speeds}
\label{fig:doppler}
\vskip -0.15in
\end{figure}


{\it FFT Bin Variation.} So far we observed frequency variation and time offset in our system design. In addition, we want to evaluate the effect of frequency shifts on assigning unique cyclic shifted chirp symbols to different \tagnames. As we mentioned before, effects of frequency offset and time offset is presented as shifts in the location of FFT peak for each transmission. Fig.\ref{fig:fft_var} shows number of FFT bin variation for different chirp bandwidth as the result of frequency and timing offset. This plot shows that as we decrease the chirp bandwidth, same FO+TO will translate to lower number of FFT bins which we also explained in theory at section XXX. Based on this results, if we want to achieve symbol error rate around 0.1\% for chirp bandwidth of 500~KHz, 250~KHz and 125~KHz we need at least 1.5, 1 and 0.8 FFT bin interval between each two adjacent transmissions.

\begin{figure}[t]
	\begin{subfigure}{\columnwidth}
    	\centering
    	\includegraphics[width=\linewidth]{./figs/7_bench_active_FO_TO/active_FOTO.eps}
		\label{fig:FOTO_passive}
	\end{subfigure}
    \vskip -0.3in
    \begin{subfigure}{\columnwidth}
    	\centering
    	\includegraphics[width=\linewidth]{./figs/7_bench_active_FO_TO/active_FO.eps}
		\label{fig:FOTO_active}
	\end{subfigure}
\vskip -0.3in
\caption{{\bf FO plus TO.} We evaluate FO plus TO for passive and active \tagnames. For active scenario, we also show the FO plus TO after adjusting FO in association phase.} 
\label{fig:FOTO}
\vskip -0.15in
\end{figure}

\subsection{Near-Far Problem}
As we discussed before, another issue that our system is facing is near-far problem. In this section, we evaluate different aspects of this problem in our system.

{\it Dynamic Range.} We evaluate dynamic range of our system in the case of multiple concurrent transmissions. To do this, we use a wired setup including two \tagnames which one is transmitting high power transmission located at the beginning of the FFT spectrum. We sweep transmission symbol on the second \tagname and decrease its power up to when we can still reliably decode chirp symbols. We show the maximum power difference of these two transmissions at each sweeping point across different cyclic shifted chirps in fig.~\ref{fig:pow_dyn}.

The results show that the maximum power difference that our system can tolerate is $\approx$35~dB and in the case of adjacent transmissions is $\approx$8~dB. Our solution to increase this dynamic range is to adjust power on the \tagname itself. For active \tagnames we do this by adjusting the power of transmissions, however on passive \tagnames we perform backscatter technique to adjust the power level. To do this, we use different backscatter constellation to decrease the power of received signal from helper and transmit packets in different power levels. We use three different power levels which they have $\approx$5~dB difference. Fig.~\ref{fig:power_spec} shows the spectrum of backscattered signal from passive \tagname at different power levels. Furthermore, fig.\ref{fig:power_fft} shows amplitude of demodulated chirp symbols after multiplying by downchirp and performing FFT operation. Spectrogram and demodulated signal show that using different power levels on passive \tagname does not change the spectrum of the signal.

\begin{figure}[t]
        \includegraphics[width=\columnwidth]{./figs/4_bench_power_dynamic/4_bench_dynamic.eps}
\vskip -0.15in
\caption{{\bf Power Dynamic Range.} We show power difference between two concurrent transmissions at different locations of FFT domain. One transmissions is static and the other is sweeping across different chirp symbols.}
\label{fig:pow_dyn}
\vskip -0.15in
\end{figure}


We evaluate our power adjustment hardware solution on passive \tagname by exploring the spectrum of of backscatter signal. We use a wired setup experiment and record backscatter signal at different power level. First, we show the FFT of demodulated signal after multiplying to downchirp symbol. Fig.~\ref{fig:power_fft} shows that by decreasing the power of signal on backscatter \tagname, FFT spectrum of demodulated signal has similar shape with lower amplitude. Also. As fig.~\ref{power_spec} shows, the spectrum of upchirp symbols at different power levels has the same properties and 

{\it Power Adjustment.} So far we show the maximum power dynamic range we can support in our system and we also evaluate our hardware solution for passive \tagname to increase power dynamic range. Next, we evaluate the effect of using power adjustment technique in our system. To do this, we setup two passive \tagnames in an office environment and transmit synchronization packets. We record packets from two \tagnames and evaluate the power difference between received signal from different \tagnames. We perform this experiment in two scenarios. First, we setup two \tagnames to use adjacent cyclic shifted chirp symbols in frequency and second we use two chirp symbols with maximum cyclic shifts. In both scenarios, we evaluate our system before and after using power adjustment technique. Fig.~\ref{fig:power_adjust} shows CDF of power difference between two transmissions in both scenarios. Maximum power difference that our system could tolerate (power threshold) for adjacent transmissions is $\approx$XX~dB and for far maximum cyclic shift is $\approx$XXX~dB. Fig.\ref{fig:power_adjust} shows that by using power adjustment method, power difference of two transmissions in both cases are less than power threshold. This shows that in cases where two transmissions have power difference more than the dynamic range, our adjustment method can improve the throughput by adjusting power of different transmissions to the dynamic power range.


\begin{figure}[t]
	\centering
    \includegraphics[width=\linewidth]{./figs/5_bench_power_adjust/bench_power_adjust.eps}
	\vskip -0.2in
	\caption{{\bf Power Adjustment Technique Evaluation.} We show CDF of power difference between two \tagname in two scenarios.}
	\label{fig:power_adjust}
\end{figure}

\begin{figure}[t]
	\begin{subfigure}{0.325\columnwidth}
    	\centering
    	\includegraphics[width=\linewidth]{./figs/2_bench_power_spec/2_bench_spec_power_high.eps}
		\label{fig:power_spec_high}
        \vskip -0.2in
        \caption{High}
	\end{subfigure}
    \begin{subfigure}{0.325\columnwidth}
    	\centering
    	\includegraphics[width=\linewidth]{./figs/2_bench_power_spec/2_bench_spec_power_med.eps}
		\label{fig:power_spec_med}
        \vskip -0.2in
        \caption{Medium}
	\end{subfigure}
    \begin{subfigure}{0.325\columnwidth}
    	\centering
    	\includegraphics[width=\linewidth]{./figs/2_bench_power_spec/2_bench_spec_power_low.eps}
		\label{fig:power_spec_low}
        \vskip -0.2in
        \caption{Low}
	\end{subfigure}
\vskip -0.1in
\caption{{\bf Spectrogram of Backscattered Signal.} We show spectrogram of received signal from passive \tagname at multiple power levels.}
\label{fig:power_spec}
\vskip -0.15in
\end{figure}






















==> existing_concurrent-1.tex <==
\section{Existing concurrent transmission CSS techniques}
In this section, we will go over different techniques that can be used to enable multiple users to transmit concurrently in the network.\par

{\bf Using Different Spreading Factors.}
If there are $N$ transmitters in the network, one way to enable concurrent transmissions is to assign different spreading factors to each of them. As shown in Fig. xx,(two upchirps with different spreading factors and their corresponding downchirps to demodulate them and the FFT results for them). There are three fundamental problems associated to this network. The first problem is, for the same $BW$ there are limited number of spreading factors that can be used that result in reason data rate and receiver sensitivity. For a LoRa protocol, this is limited 7 different spreading factors. Second, the receiver needs to use downchirps with different spreading factors to despread upchirp symbols of different transmitters which increases the receiver complexity. Third, upchirps with different spreading factors are not orthogonal. As shown in Fig. xx(figure with upchirps with different spreading factors and their despread version and noise contributions), if we have a signal composed of two upchirps with different spreading factors and we despread this signal using the downchirp corresponding to first upchirp, then the second upchirp will increase the noise floor of the first upchirp. This will reduce the sensitivity of the receiver. \par

{\bf CHOIR.} 
Imagine that there are two perfectly synchronized transmitters sending two different upchirp symbols as shown in Fig. xx a (two different upchirps with different colors in one figure). By superposition theorem, we will be able to see two different peaks in the FFT of the received signal shown in Fig. xx b. In particular, if we are able to: 1- differentiate these peaks and 2- associate them to the corresponding transmitter 3- Be sure that they do not use the same FFT bin at the same time, we can have a network that supports multiple transmitters. One way to differentiate between the transmitters is to use the fraction in their FFT peak indexes(cite CMU paper). However, this is limited to 10 in an ideal case. More importantly, if there are $N<11$ transmitters in the network, the probability for these transmitters having different FFT peak index fractions is equal to:
\begin{equation}
P_{Different Fraction}=\frac{10!}{(10-N)!10^N}
\end{equation}\par
To make sense of the above probability if $N=5$, this probability would be 30\% which is unpractical. Moreover, if these two transmitters use the same upchirp symbol at the same time, it will result in a collision that cannot be decoded. In the case of LoRa modulation, if there are $N$ transmitters and assuming random symbols at each symbol time interval, the probability of collision is equal to:
\begin{equation}
P_{collision}=1-\prod_{i=1}^{N}(1-\frac{i}{2^{SF}})\simeq\frac{N(N+1)}{2^{SF+1}}
\end{equation}\par
Assume $SF=9$ and $N=10$, collision probability is approximately 10\% in this case. In the next section, we go over the \nameshort and explain how it will satisfy the three requirements mentioned above.


==> existing_concurrent.tex <==
\section{Existing concurrent transmission CSS techniques}
In this section, we will go over different techniques that can be used to enable multiple users to transmit concurrently in the network.\par

{\bf Using Different Spreading Factors.}
If there are $N$ transmitters in the network, one way to enable concurrent transmissions is to assign different spreading factors to each of them. As shown in Fig. xx,(two upchirps with different spreading factors and their corresponding downchirps to demodulate them and the FFT results for them). There are three fundamental problems associated to this network. The first problem is, for the same $BW$ there are limited number of spreading factors that can be used that result in reason data rate and receiver sensitivity. For a LoRa protocol, this is limited 7 different spreading factors. Second, the receiver needs to use downchirps with different spreading factors to despread upchirp symbols of different transmitters which increases the receiver complexity. Third, upchirps with different spreading factors are not orthogonal. As shown in Fig. xx(figure with upchirps with different spreading factors and their despread version and noise contributions), if we have a signal composed of two upchirps with different spreading factors and we despread this signal using the downchirp corresponding to first upchirp, then the second upchirp will increase the noise floor of the first upchirp. This will reduce the sensitivity of the receiver. \par

{\bf CHOIR.} 
Imagine that there are two perfectly synchronized transmitters sending two different upchirp symbols as shown in Fig. xx a (two different upchirps with different colors in one figure). By superposition theorem, we will be able to see two different peaks in the FFT of the received signal shown in Fig. xx b. In particular, if we are able to: 1- differentiate these peaks and 2- associate them to the corresponding transmitter 3- Be sure that they do not use the same FFT bin at the same time, we can have a network that supports multiple transmitters. One way to differentiate between the transmitters is to use the fraction in their FFT peak indexes(cite CMU paper). However, this is limited to 10 in an ideal case. More importantly, if there are $N<11$ transmitters in the network, the probability for these transmitters having different FFT peak index fractions is equal to:
\begin{equation}
P_{Different Fraction}=\frac{10!}{(10-N)!10^N}
\end{equation}\par
To make sense of the above probability if $N=5$, this probability would be 30\% which is unpractical. Moreover, if these two transmitters use the same upchirp symbol at the same time, it will result in a collision that cannot be decoded. In the case of LoRa modulation, if there are $N$ transmitters and assuming random symbols at each symbol time interval, the probability of collision is equal to:
\begin{equation}
P_{collision}=1-\prod_{i=1}^{N}(1-\frac{i}{2^{SF}})\simeq\frac{N(N+1)}{2^{SF+1}}
\end{equation}\par
Assume $SF=9$ and $N=10$, collision probability is approximately 10\% in this case. In the next section, we go over the \nameshort and explain how it will satisfy the three requirements mentioned above.












==> network_communication_protocol.tex <==
\section{Network protocol}
In this section, we will go over synchronization, network association, communication and also how do we support more number of users that a band can support in the same bandwidth with TDMA.

\subsection{Synchronization and Synchronization Packet}
As explained previously, we need to synchronize all the \tagnames using the synchronization packet sent by the reader. 
Synchronization packet conveys information regarding cyclic shift assignment and scheduling assignment for a \tagname who is in association process. It also has the information regarding which timing schedule are we in as explained in Section ~\ref{schedule}. In addition to that, \tagnames who are in association phase use this packet's RSSI for two purposes: i) they will coarsely localize themselves to compensate for their $ToF$ delay and ii) adjust their transmit power.\par
\subsection{Network Association}\label{assoc}
Assume that a network of $N$ \tagnames are communicating to the reader and the $(N+1)th$ \tagname wants to associate with the network. We can imagine two ways of doing this. One way is to set time intervals of communication phase different from those of association phase. This can be done by making synchronization packets sent by the reader for communication different from the ones sent by it for association so that the \tagnames who want to enter the network listen to association packets and the ones who are already in the network and want to communicate listen to synchronization ones. However, this method would cause high latency in the network. The second way is to assign ?? number of cyclic shifts and hence FFT bins for association and the rest for communication. In this case, communication synchronization packet and association are the same. In other words, all the \tagnames transmit at the same time but the ones who want to enter the network transmit in association cyclic shifts and after finishing the association process, they use the communication cyclic shifts. This way, the association latency will be lower than the previous case. Three questions should be answered regarding this method.\par
First, which cyclic shifts are assigned to association and which are for communication? As explained in the Near-Far Problem in Section ~\ref{issue}, to get the maximum dynamic range, adjacent cyclic shifts are assigned to \tagnames with small power differences. In this case, if the association cyclic shifts are the low power ones and the incoming device is high power, it can overpower the existing \tagnames in the network and if it is in high power FFT bin interval, it can be drowned. To solve this, we provisioned two cyclic shift intervals, one in high power and the other one in low power cyclic shift regions. The incoming \tagname would choose which association region to transmit based on the synchronization packet's RSSI.\par
Second, how many cyclic shifts, $k_{assoc.}$, should we put aside for association? We set this network parameter based on the frequency and timing offsets that cannot be compensated by the \tagname. As explained in Section ~\ref{issue}, hardware delay variations are dealt with using the empty cyclic shifts. The same method can be used here to make sure that we are not missing any incoming \tagname. \par
The last question is, what happens if more than one \tagname want to associate at the same time? To solve this, we can use slotted-Aloha based scheduling and provision more association cyclic shifts in both high power and low power regions to enable more users to associate at the same time.\par
After the \tagname sent packet to the reader in the association cyclic shifts, the reader finds this packet's RSSI and decides which cyclic shift it should be assigned to. In the next synchronization process, the reader will send the assigned cyclic shift along with the \tagname's scheduling in the synchronization packet. The \tagnames who are already in the network discard the assigned cyclic shift and scheduling information and the incoming \tagnames use this information and communicate in that cyclic shift in the next communication cycle.

\subsection{Communication and Receiver} 
In communication phase, after receiving the synchronization packet, all the \tagnames who are already in the network will start transmitting packets in the communication cyclic shifts.
{\it Packet Structure.}
The \tagname packet structure is shown in Fig. ~\ref{packet_structure} (figure showing packet structure which consists of upchirp and downchirp preambles and the payload). 
The packet starts with upchirp and downchirp preambles. They are designed to serve two purposes: i) finding the start of the packet ii) detecting the transmissions. We need to emphasize here that the \tagname uses its assigned code for preamble for both upchirp and downchirp and also for payload. As shown Fig. ~\ref{time_domain_chirp_sequence}(2 time domain chirp sequences corresponding to two different devices so that it shows what do we mean by having the downchirp code the same as upchirp. Mark the upchirp trip point and downchirp trip point, to explain why the difference will result in the assigned code). Preamble consists of $6$ number of $1$s which follows by $2$ downchirps. What comes after is the payloads. 

{\it Finding The Start of The Packet.}
Consider the Fig. ~\ref{time_domain_chirp_sequence} a, since the upchirp code is the same as downchirp code, if we find the start of the last upchirp symbol, point $P_{1}$, and also the end of the first downchirp symbol in preamble, point $P_{2}$, we can find the middle point of these two points, point $P_{M}$, which corresponds to the end of the upchirp preambles. Now, we can go back $6$ preamble durations and find the start of the packet. Notice that $P_{M}$ does not rely on frequency offset because of the symmetry that is designed in upchirp and downchirp codes. How can we find $P_{1}$ and $P_{2}$? As shown in Fig. ~\ref{upchirp_sweep} $P_{1}$ can be found by time domain sweeping and multiplying the signal by the baseline downchirp and taking FFT. Doing this we can find the time that the FFT bin peak index changes from the maximum to minimum, called trip point, or upchirp's instantaneous frequency changes from $\frac{BW}{2}$ to $-\frac{BW}{2}$. If we find the last time that this happens we can find the start of the last upchirp symbol in preamble. The same sweep can be done in the preamble downchirp symbols to find the end of the first downchirp by sweeping the baseline upchirp. To make both of these time domain sweepings more efficient, we can start with a high sweep step size and decrease it as we get closer to the target trip point.

{\it Transmission Detection.} 
Now that we found the start of the packet, we need to find out which transmitters are in the network. To do so, for each preamble upchirp symbol, we demodulate it and look at the peaks in FFT domain. If there is an FFT peak index in the demodulation results of all the preamble symbols consistently and the power of that FFT peak is more than the threshold determined by the power of high power \tagnames' indexes, we realize that the \tagname corresponding to that FFT bin is sending data. After finding these indexes, we can find the average power over the $6$ preambles for each of these FFT bins. This average power can be used as a threshold to determine if each \tagname is sending $0$ or $1$ at each of its payload symbols. In particular, if the power of the \tagname's corresponding FFT bin for each payload symbol is more than half this average, we interpret that as $1$ and otherwise $0$.
\subsection{Scheduling More \tagNames}\label{schedule}
In this part, we answer this question, that what happens if we want to support more \tagnames that one band can support using only one band. The assumption here is that we know the duty-cycle of the network. As mentioned in Section ~\ref{assoc}, there are two assignments happening in the association phase: i)cyclic shift ii)scheduling. Assuming duty-cycle of the network is $1\%$, in this case there are $100$ different timing schedules that in each of them a group of \tagnames will transmit concurrently. In this example, there are 100 different synchronization packets corresponding to each timing schedule. After receiving the synchronization packet, the \tagname will check if it corresponds to its scheduling or not. If yes, it starts transmitting in the coming communication cycle.













==> overview.tex <==
\section{System Design}
We use backscatter to transform transmissions from Bluetooth devices into Wi-Fi signals. In this section, we first provide an overview of Bluetooth and Wi-Fi physical layers and then describe how to create single-tone transmissions using Bluetooth devices. We then show how to create an 802.11b signal from this single tone Bluetooth transmission. Finally, we outline our design for bi-directional communication using OFDM Wi-Fi as an AM modulator.



==> practical_issues.tex <==
\section{Practical Issues}
As explained in previous sections, in DCSS, we assign different cyclically shifted chirps and hence FFT bins to different \tagnames in the network and each modulates its data by doing ON-OFF keying. There three practical issues associated with the above modulation:\par
{\bf Timing Mismatch.} The above design requires all the \tagnames to be time synchronized. To understand why, assume that two consecutive baseline upchirs are being (Fig. ~\ref{fig:timing_offset}). If we consider the blue or red timing interval as chirp symbol interval we will get different FFT bin peak index locations and can misinterpret its corresponding \tagname. This means, with $\Delta t$ timing mismatch, the corresponding FFT bin and hence its associated \tagname would change by :
\begin{equation}\label{fft_delay_var}
FFT_{var}=\Delta t BW
\end{equation}\par
As a result, all the \tagnames in the network should be synchronized. To do so, the reader sends synchronization packet \tagnames and after this packet is received and processed by the \tagnames, they start transmitting. However, there are two kinds of delay in the network. First, since \tagnames can have different distances from the reader, the time of flight ($ToF$) delay of them would be different. Moreover, \tagnames have hardware variations and this will cause them to start transmitting in different time instances. The source of these hardware delay variations come from the fact that the envelope detector which receives the synchronization packets and the communication between this module and chirp transmitter have variations. This causes the delay to change from packet to packet.\par
Passive \tagnames are mostly used in relatively small areas, $d<100m$, which translates to $ToF<333nS$. This delay in turn will translate to $0.16$ FFT bin change, assuming $BW=500 KHz$. However, as shown Evaluation Section ??, the hardware delay variation and hence its corresponding FFT bin change can be be higher and go over one FFT bin. This means that the signal transmitted by one \tagname can be interpreted as a signal transmitted from the adjacent \tagname. The way to get around this problem is to put some number of empty FFT bins adjacent to each FFT bin assigned to an \tagname. The reason is that this delay would change over time and from packet to packet In other words, if FFT bin $N_{1}$ is assigned to \tagname 1, the adjacent $k$ FFT bins are empty and not assigned to any \tagname. Doing so, reduces the chances of misinterpretation significantly, as shown in Evaluation Section. Considering equation ~\ref{fft_delay_var}, $k$ can be determined knowing the chirp $BW$ and hardware delay variations. Since, the latter is nearly constant with $BW$, decreasing the $BW$ will decrease the required $k$.\par
The case is different for active \tagnames since in addition to the hardware delay, they can be as far as $10km$ which translates to $16.7$ FFT bin change, considering the $BW=500 KHz$. To solve this problem, reader will coarsely localize the active \tagname using its received packet's RSSI and then change the starting time of the other \tagnames to change their starting time in such a way that all of the \tagnames' packets is received by the receiver at the same. Localization accuracy needed for this delay correction is $d<100m$ since it translates $FFT_{var}<0.16$ which will make sure that one \tagname will not be mistaken by the adjacent one.\par

{\bf Frequency Offset.} 
\tagnames experience different frequency offsets because of hardware variations in the crystals used in their oscillators. As explained in Section ~\ref{css_primer}, change in frequency translates to FFT bin change of the demodulated \tagname packet. This again, causes that one \tagname being misinterpreted as other \tagname. For frequency change of $\Delta f$, the $FFT_{var}$ can be written: 
\begin{equation}\label{fft_freq_var}
FFT_{var}=\frac{\Delta f}{\frac{BW}{2^{SF}}}
\end{equation}\par
Crystals' frequency tolerance can be as high as $100ppm$. Considering that passive \tagnames run at a few MHz frequencies, this frequency variation translates to less than one FFT bin for $BW=500KHz$ for most of the $SF$s as evaluated in Section ~\ref{eval}. On the other hand, active \tagnames experience much higher frequency variations since they generate frequencies at UHF band. This frequency variation translates to multiple FFT bins. The solution to this problem is that the reader finds the frequency offset and communicates that to \tagname in network association phase. Then, the \tagname will adjust its frequency in a way that the net result would be its assigned FFT bin.\par

{\bf Near-Far Problem.}
Having a network of multiple concurrent transmissions, the power of far or lower power \tagnames can be drowned in high power or close ones. In particular, if there is a single \tagname in the network and it is assigned FFT bin is $N_{1}$, the FFT side-lobe powers of this system is shown in Fig. ~\ref{fft_ideal_side_lobe}. Now, if there is a second \tagname in the network with assigned FFT bin of $N_{2}$ and its power is lower than the power of side-lobes of the first transmitter at $N_{2}$ FFT bin, it cannot be decoded. This suggests that, we should assign the adjacent FFT bins to \tagnames that have small power difference. In that case, low power \tagnames will be far from high power ones in FFT domain and can be decoded less error despite having low power. Section ~\ref{eval} evaluates this method.\par
The second method is adjust and bring down the power of high power \tagnames in association phase. Doing this, we will be able to decode packets having even lower power that Fig. ~\ref{fft_ideal_side_lobe} and Section ~\ref{eval} suggests. 















==> receiver.tex <==
\section{Receiver Design}

Points:
Explain receiver design
Explain the high FFT size and zero-padding
How to find the start of the packet
Upchirp sweep
downchirp sweep
detect preamble values
Find expected symbol
How do we deal with false positive? => thresholding
How do we differentiate between 0 and 1?
Using the threshold that we find in preambles 


This section describes how MU-CSS can decode concurrent CSS transmissions which utilize same frequency spectrum. Detecting the beginning of the transmission is a key factor in decoding transmissions. Our receiver takes several steps to detect a transmissions, synchronize in time domain and differentiate the frequency of each transmission.

{\bf Detecting a Transmission}. Our detection mechanism is based on energy detection technique using CSS. Specifically, receiver is looking for finding similar chirp symbols in received signal. Therefore, we multiply time-domain signal with a baseline downchirp, then perform an FFT operation and find the maximum. By detecting multiple chirp symbols with same FFT value, receiver detects the energy of the preamble which is the starting point of the transmission.

{\bf Time Synchronization}. As mentioned before, timing offset on a chirp symbol translates to frequency shift in demodulated symbol. Time synchronization to needs to be really accurate to demodulate a chirp symbol. Demodulating a single CSS transmission is trivial, because receiver knows value of preamble symbols. This become more complicated when there are multiple CSS transmissions and each has different preamble symbols. We take advantage of two key parts of our CSS transmissions to time synchronize the receiver with transmissions.
As we mentioned the packet structure in section \ref{packet_structure_section}, each packets start with preamble including multiple upchirp symbols which has the same value. Following the preamble, there are two and a quarter downchirp symbols which also has same value as preamble symbols. The key idea is to find three points in the transmission as fig.~\ref{fig:trip_points} shows, which leads to time synchronization. Regardless of the transmission symbol value, these three points exist on every transmission. Point A shows the last trip point in preamble section, point B shows the first trip point in downchirp symbols and point C shows the starting point of downchirp symbols. Detecting points A and B leads to detection of point C which is the middle point of A and B. Also, distance between A and B in time-domain signal is a function of transmission chirp symbol value. We use time-domain sweeping technique to detect A and B which we describe in following sections.

{\bf Time-Domain Sweeping}. The goal of the time-domain sweeping on CSS transmission is to determine a location in a CSS transmission where chirp symbol is aliasing. We call these locations trip points as fig.~\ref{fig:trip_points} shows. Time-domain sweeping perform as following: we multiply a baseline downchirp symbol with received upchirp symbols. By applying FFT on the result we can find the location of the peak in FFT domain. Then, we sweep the baseline downchirp symbol by one sample and perform these operations again to get another peak in FFT domain. As we sweep across the the received signal and because there are multiple 

Continue this!

that distance between starting point of the last upchirp symbol and starting point of downchirp symbols is a function of the symbol value and it is unique for each transmission.

Sweeping technique
key idea of decoding a multiple CSS transmission is that the receiver needs to be exactly synchronized to the starting point of the packet.


\subsection{Detecting Transmissions}




